Discrimination in the Venture Capital Industry: Evidence from Field Experiments

This paper examines discrimination by early-stage investors based on startup founders' gender and race using two complementary field experiments with real U.S. venture capitalists. Results show the following. (i) Discrimination varies depending on the context. Investors implicitly discriminate against female and Asian founders when evaluating attractive startups, but they favor female and Asian founders when evaluating struggling startups. This helps to reconcile the contradictory results in the extant literature and confirms the theoretical predictions of "discrimination reversion" and "pro-cyclical discrimination" phenomena. (ii) Among multiple coexisting sources of discrimination identified, statistical discrimination and implicit discrimination are important reasons for investors' "anti-minority" behaviors. A consistent estimator is developed to measure the polarization of investors' discrimination behaviors and their separate driving forces. (iii) Homophily exists when investors provide anonymous encouragement to startups in a non-investment setting. (iv) There was temporary, stronger discrimination against Asian founders during the COVID-19 outbreak.

==> backup.tex <==
\begin{center}
\begin{table}
 \caption{Experiment A Implicit discrimination Based on Founder's Race by Investors' Contact Interest}
  \label{implicit bias race stake}

\begin{tabular}{m{6cm} c c c c c c} 
\toprule
Dependent Variable&Response Time&Q1&Q2&Q3&Q4&Q5\\
&(Unit: Second)&Quality&Availability&Contact&Investment&Risk\\
&(1)&(2)&(3)&(4)&(5)&(6)\\
\midrule
\emph{Panel A: Contact Interest is High}&&&&&&\\
\emph{($Q3>=50$)}&&&&&&\\
&&&&&&\\
Second Half of Study&-28.05***&	4.85**&	-0.43&	1.83&	0.90***&	-3.63\\
&(3.00)&	(1.88)&	(1.16)&	(1.41)&	(0.33)&	(4.60)\\
Asian Founder&-0.58&	3.51*&	-1.36&	0.92&	0.58*&	-1.08\\
&(3.15)&(1.95)&	(1.33)&	(1.57)&	(0.35)&	(5.55)\\
Asian Founder $\times$&&-7.94***&0.02&	-3.66*&	-1.44***&	6.56\\
Second Half of Study&&(2.76)&	(1.79)&	(2.20)&	(0.51)&	(7.23)\\
&&&&&&\\
p-value of Asian Founder in&&0.02&0.25&0.06&0.01&0.25\\
the second half of study&&&&&&\\
Investor FE &Yes&Yes&Yes&Yes&Yes&Yes\\
Observations&724&724&692&724&698&127\\
R-squared&0.37&	0.41&	0.68&	0.44&	0.45&	0.20\\
&&&&&&\\
&&&&&&\\
\emph{Panel B: Ivy-scaled Coefficient}&&&&&&\\
(In the Second Half of Study)&&&&&&\\
&&&&&&\\
Ivy League College&&8.78***&-0.48&	8.65***&1.20***&-10.69**\\
&&(1.67)&(1.12)&(1.96)&(0.31)&(4.17)\\
Asian Founder/Ivy League College&&-0.49& 1.27& -0.38& -0.80& -0.36\\
&&&&&\\
&&&&&\\
\emph{Panel C: Contact Interest is Low}&&&&&\\
\emph{($Q3<50$)}&&&&&&\\
&&&&&&\\
Second Half of Study&-26.46***&	1.90&	3.62&	2.33*&	1.07***	&-1.73\\
&(3.91)&(1.86)&	(2.20)&	(1.39)&	(0.27)&	(4.00)\\
Asian Founder&2.11&	1.91&	1.57&	2.73*&	0.47&	-4.57\\
&(3.90)&(1.82)&	(2.32)&	(1.61)&	(0.30)&	(4.15)\\
Asian Founder $\times$&&-1.26&	-3.13&	-2.48&	-0.22&	8.46\\
Second Half of Study&&(2.68)&(3.08)&	(2.09)&	(0.42)&	(6.19)\\
&&&&&&\\
p-value of Asian Founder in&&0.72&0.44&0.85&0.39&0.33\\
the second half of study&&&&&&\\
Investor FE &Yes&Yes&Yes&Yes&Yes&Yes\\
Observations&492&492&492&492&478&49\\
R-squared&0.33&	0.48&	0.60&	0.50&	0.62&	0.87\\
\bottomrule
\end{tabular}
\end{table}
\end{center}


\clearpage
\begin{center}
\begin{table}
\begin{tablenotes}
 \item \emph{Notes.} This table reports regression results of how investors' response time and evaluation results respond to a startup founder's race in the ``high contact interest" situations and the ``low contact interest" situations. Panel A tests the implicit racial discrimination in the ``high contact interest" situations in which investors' contact interest is higher than or equal to 50\% probability. Panel B calculates the relative magnitude of the implicit racial discrimination in ``high contact interest" situations compared with the effect of going to an Ivy League college by using the profiles in the second half of the study. Panel C tests the implicit racial discrimination in the ``low contact interest" situations in which investors' contact interest is lower than 50\% probability. Results are similar if I choose other thresholds like 40\% or 45\%. ``Asian Founder" is a dummy variable that is equal to one if the startup founder has an Asian last name, and zero otherwise. ``Ivy League College" is a dummy variable that is equal to one if the startup founder graduates from an Ivy League college, and zero otherwise. ``Second Half of Study" is an indicator variable for startup profiles shown among the last eight resumes viewed by a subject. In Column (1), the dependent variable is investors' response time, which is defined as the number of seconds before each page submission, winsorized at the 95th percentile (59.23 seconds on average). Columns (2)-(6) show the quality evaluation, availability evaluation, contact interest, investment interest and risk evaluation separately. Results are still robust when clustering standard errors on the investor level. ***$p<0.01$, **$p <0.05$, *$p<0.1$
\end{tablenotes}
\end{table}
\end{center}

